Sketch In, Sketch Out: Accelerating both Learning and Inference for Structured Prediction with Kernels

Leveraging the kernel trick in both the input and output spaces, surrogate kernel methods are a flexible and theoretically grounded solution to structured output prediction. If they provide state-of-the-art performance on complex data sets of moderate size (e.g., in chemoinformatics), these approaches however fail to scale. We propose to equip surrogate kernel methods with sketching-based approximations, applied to both the input and output feature maps. We prove excess risk bounds on the original structured prediction problem, showing how to attain close-to-optimal rates with a reduced sketch size that depends on the eigendecay of the input/output covariance operators. From a computational perspective, we show that the two approximations have distinct but complementary impacts: sketching the input kernel mostly reduces training time, while sketching the output kernel decreases the inference time. Empirically, our approach is shown to scale, achieving state-of-the-art performance on benchmark data sets where non-sketched methods are intractable.

==> 100-notes_lbm.tex <==
\section{Recall methods}

\paragraph{Goal. } In order to reduce the computational cost of training we propose to sketch the input kernel. In order to reduce the computational cost of decoding (pre-image) we propose to sketch the output kernel. This consists in randomly projecting the input and output kernels' feature maps on random linear subspaces.

\paragraph{Sketching method. } The sketching method consists in approximating a feature map $\chi : \bmZ \to \bmH_z$ by projecting it thanks to a random projection operator $\widetilde P_Z \in \bmH_z \otimes \bmH_z$ defined as follows. Given a random matrix $R_z \in \reals^{m \times n}$ and $n$ data $(z_i)_{i=1}^n \in \bmZ$, the linear subspace defining $\widetilde P_Z$ is constructed as the linear subspace generated by the span of the following $m$ random vectors
\begin{align}
    \sum_{j=1}^n (R_z)_{ij} \chi(z_j) \in \bmH_z, \quad i=1, \dots, m.
\end{align}
The resulting approximated feature map is
\begin{align}
    \tilde \chi(z) = \widetilde P_Z  \chi(z).
\end{align}


\paragraph{Ridge estimator. } The ridge estimator writes as
\begin{align}
    \hat h(x) = \hat H \phi(x)
\end{align}
with
\begin{align}
    \hat H = S_Y^{\#}S_X(S_X^\# S_X + \lambda I_{\bmH_x})^{-1}
\end{align}


\paragraph{Approximated ridge estimator. }  We use sketching for approximating both the input and the output feature maps. The proposed approximated estimator writes as
\begin{align}
    \tilde h(x) = \tilde H \phi(x)
\end{align}
with
\begin{align}
    \tilde H &= P_Y S_Y^{\#}S_X P_X(P S_X^\# S_X P + \lambda I_{\bmH_x})^{-1}\\
    &= P_Y S_Y^{\#}S_X VV^\#(VV^\# S_X^\# S_X VV^\# + \lambda I_{\bmH_x})^{-1}\\
    &= P_Y S_Y^{\#}S_X V (V^\# \hat C_X V + \lambda I_{\bmH_x})^{-1}V^\#\\
    &= P_Y S_Y^{\#}S_X \tilde{\eta}(\widehat{C}_X)
\end{align}
using the so-called push-through identity $(I + UV)^{-1}U = U(I + VU)^{-1}$.

% {\color{teal}
% En fait je retrouve bien ce que j'ai trouvé au lemme 2, faut juste utiliser le fait que $V^{\#} V = I_{p_x}$ à la dernière ligne
% \begin{align*}
%     \tilde H &= P_Y S_Y^{\#}S_X P_X(P S_X^\# S_X P + \lambda I_{\bmH_x})^{-1} \\
%     &= P_Y S_Y^{\#}S_X VV^\#(VV^\# S_X^\# S_X VV^\# + \lambda I_{\bmH_x})^{-1} \\
%     &= P_Y S_Y^{\#}S_X V (V^\# VV^\# \hat C_X V + \lambda I_{\bmH_x})^{-1}V^\# \\
%     &= P_Y S_Y^{\#}S_X V (V^\# \hat C_X V + \lambda I_{\bmH_x})^{-1}V^\#\,.
% \end{align*}
% Après pour la partie algo, faudra juste faire l'inverse que ce que je fais dans le lemme 2 pour identifier ce que ça donne comme $\alpha$.
% }

\paragraph{Algorithm. } Finally, in practice, it is possible to compute for any $y \in \bmY$ the quantities $\langle \tilde h(x), \, \psi(y)\rangle_{\bmH_y}$, as follows. We have
\begin{align}
    \tilde h(x) = \sum_{i=1}^n \tilde \alpha_i(x) \tilde P_Y \psi(y_i)
\end{align}
where $\tilde \alpha_(x) = ...$ (the one given above). Moreover, one can compute the following scalar products as follows
\begin{align}
    \langle \tilde h(x), \, \psi(y)\rangle_{\bmH_y} &= \sum_{i=1}^n \tilde \alpha_i(x) \langle \tilde P_Y \psi(y_i), \psi(y)\rangle_{\bmH_y}\\
    &= ...
\end{align}





\paragraph{$P_Z$ expression. } By definition
\begin{align}
    P_Z = VV^{\#}
\end{align}
where $U\Sigma V^{\#}$ is the SVD of $R_zS_Z \in \reals^m \otimes \bmH_z$.
It can be also be shown that
\begin{equation}
    \widetilde{P}_Z = n S_Z^{\#} R_z^\top \widetilde{K}_Z^\dagger R_z S_Z = (R_z S_Z)^{\#} \left(R_z S_Z (R_z S_Z)^{\#}\right)^{\dagger} R_z S_Z\,.
\end{equation}


























==> 200-model-old.tex <==
\section{Problem Setting and Sketched Estimators}
\label{sec:model}
\fl{Proposition for the presentation:} \\

\begin{itemize}
\item Structured prediction problem setting
\item Surrogate  methods with their nice features and IOKR-ridge as an emblematic surrogate method to solve SP
(with an introduction of notations and the closed form with sampling operators..)
\item Incentives to approximate both input and output (training / inference)
\item Focus on sketching as random projection  + state of the art and thought path:= what has been proposed below by Pierre 1-to-4 to make this approximation 
\end{itemize}
I would then announce  the steps we'll have to take:
\begin{enumerate}
\item SISOKR and theoretical guarantees, including sketching approximation error (section 3)
\item then Sketched SP: $\widetilde f$ that benefits i) from usual theoretical guarantees due to those of $\widetilde{h}$ and reduced computational cost (section 4)
\end{enumerate}

\fl{end of proposition}


Proposition to introduce sketching:
%
\begin{enumerate}
\item Ridge regression without sketching \pl{maybe not even necessary if already discussed before}
%
\item Sketched Ridge regression through the change of variable $\alpha = R^\top \gamma$, see \citep[Section~2.2]{Yang2017} in the scalar case. But not easy to generalize to vv-outputs \pl{@Tamim, what's the reason exactly, a gradient problem right?}
%
\item Sketching also amounts to minimize over the projected subspace, see \citep[Proposition~2]{Yang_NIPS2012_621bf66d} for Nystr\"{o}m's method on scalar outputs, and \citep[Proposition~5]{elahmad22} for a generalization to any sketch matrix and (finite-dimensional) vector-valued outputs. But impractical with vv-outputs \pl{@Tamim, same question as above}
%
\item Minimizing on the projected subspace is equivalent to replace $S_X$ with $S_X \widetilde{P}_X$ in the closed-form solution, see \citep[Lemma~1]{rudi2015less} for Nystr\"{o}m's method on scalar-valued outputs .
\end{enumerate}
%
We propose to extend the latter view to vv-outputs, and to use it on both $S_X$ and $S_Y^\#$ in the closed-form solution $\hat{h}(x) = S_Y^\# S_X \big(\widehat{C}_X + \lambda I\big)^{-1} \phi(x)$ from \citep[Lemma~17]{Ciliberto2016}

% \lbm{As said in our previous meeting I like the version 4. This is also true for the output projection. Minimizing on $\tilde \bmH = \widetilde P_y \bmH_y \otimes \widetilde P_x \bmH_x$ is equivalent to replace $S_Y$ with $S_Y \widetilde{P}_Y$ in the closed-form solution. Another possibility could be to directly say that we approximate $S_X^T, S_Y^T$ by $P_X S_X^T, P_Y S_Y^T$ in the closed-form of the ridge. Finally, because the closed-form solution is a standard result from the literature of least-squares (\citep[Lemma~17]{Ciliberto2016} just extend it to infinite dimensional output space), I would say: ... in the closed-form solution of the ridge estimator $\hat h(x) = ...$ (\citep[Lemma~17][See]{Ciliberto2016})}


In this section, we present a model to tackle structured prediction problems -- Input Output Kernel Regression (IOKR) -- as well as how we leverage sketching approximation to accelerate this model in both learning and inference phases.
%

\subsection{Structured Prediction and Output Kernel Regression}

Structured prediction consists in solving a supervised learning task where the output variable is a structured object (e.g., sequences, images, graphs). Denoting $\mathcal{X}$ the input space and $\mathcal{Y}$ the structured output space, the goal is to estimate a function $f: \mathcal{X} \rightarrow \mathcal{Y}$ thanks to a finite set of observations $\left(x_i, y_i\right)_{i=1}^n$ independently drawn from an unknown distribution $\rho$ on $\mathcal{X} \times \mathcal{Y}$. The target $f^*$ is defined as
\begin{equation}\label{eq:struct_pb}
    f^*=\underset{f: \mathcal{X} \rightarrow \mathcal{Y}}{\arg \min } ~ \mathbb{E}_\rho \left[\Delta(f(x), y)\right]\,,
\end{equation}
where $\Delta: \mathcal{Y} \times \mathcal{Y} \rightarrow \reals$ is a chosen structured loss function. \\ \\
%
A standard learning approach is to define the estimator $\hat{f}$ as minimizing the empirical risk
\begin{equation}\label{eq:struct_pb_emp}
    \hat{f}=\underset{f \in \mathcal{F}}{\arg \min } ~ \frac{1}{n} \sum_{i=1}^n \Delta\left(f\left(x_i\right), y_i\right)\,,
\end{equation}
where $\mathcal{F}$ is a chosen set of hypothesis functions. In structured prediction, because $\mathcal{Y}$ is not a linear space, empirical risk minimization approach causes both modeling and computational challenges. Indeed, how to design $\mathcal{F}$ such that for all $x \in \mathcal{X}$ and $f \in \mathcal{F}$ we have $f(x) \in \mathcal{Y}$? Most methods consider $f$ of the form $f(x)=$ $\arg \max _{y \in Y} F(x, y)$ where $F$ is a score function from $\mathcal{X} \times \mathcal{Y}$ to $\reals$ (see e.g., \citet{belanger2016structured, tsochantaridis2004, nowozin2011}). Because of the $\argmax$, computing $\hat{f}$ by solving \eqref{eq:struct_pb_emp} can be very hard. \\ \\
%

\fl{meme pour une loss ILE, l'espace de Hilbert de sortie implicite n'est pas nécessairement un RKHS- dans le cas des sorties RKHS, on definit a priori un noyau - et puis ta presenattion est trompeuse ce n'est pas Ciliberto qui a introduit cela}
To build $\hat{f}$, we consider the family of methods called surrogate methods \citep{Ciliberto2016, ciliberto2020general}.
%\paragraph{Surrogate methods.} We consider the following family of methods for building $\hat{f}$.
Let $\psi: \mathcal{Y} \rightarrow \bmH_y$ be an embedding map, such that $\bmH_y$ is a separable Hilbert space called the embedding space. The decision function $\hat{f}$ is defined as follows.
\begin{enumerate}
    \item $\hat{h}$ estimates $h^*=\underset{h : \mathcal{X} \rightarrow \bmH_y}{\arg \min } ~ \mathbb{E}\left[\left\|h\left(x_i\right)-\psi\left(y_i\right)\right\|_{\bmH_y}^2\right]$ (fitting step).
    \item $\hat{f}(x)=\arg \min _{y \in \mathcal{Y}}\|\hat{h}(x)-\psi(y)\|_{\bmH_y}^2$ (decoding step).
\end{enumerate}
%
Interestingly, for any positive definite kernel $k_y: \mathcal{Y} \times \mathcal{Y} \rightarrow \reals, \psi$ can be defined as $\psi(y)=k_y(y,\cdot) \in \mathcal{H}_y$, noting $\mathcal{H}_y$ the associated Reproducing Kernel Hilbert Space (RKHS). This choice of output embedding is called Output Kernel Regression (OKR) \citep{westonNIPS2002, geurts2006, Kadri_icml2013}.
%
\fl{Presentation utile au papier:}
\subsection{Notations}
$\bmF (\bmX, \bmY)$ denoting the set of functions from $\bmX$ to $\bmY$.



\paragraph{Structured Output Prediction with kernels. }  Let $\bmX$ be the input space and $\bmY$, the output space. We consider that the elements of $\bmY$ possess some structure, e.g. they are composed of different components that interact with each other. In many cases, $\bmY$ is finite, extremely large and does not enjoy the usual wishable properties of an Euclidean space. As a consequence the supervised learning task that consists of approximating the relationship between a random variable $Y$ with values in $\bmY$ from an input variable $X$ with values in $\bmX$ requires some relaxation to be tractable \cite{nowozin2011}. In this work, we rely on kernels and infinite dimensional embeddings to overcome this issue.

Suppose a positive definite kernel $k_{y}:\bmY \times \bmY \to \reals$ that measures how close are two objects from $\bmY$. Typically $k_y$ can be chosen among the numerous kernels between complex objects reported in the literature \citep{Gartner08}. Denote $\bmH_y$ the Reproducing Kernel Hilbert Space associated to $k_y$ and $\psi: \bmY \to \bmH_y$, the canonical feature map such as $\psi(y):= k_y(\cdot,y), \forall y \in \bmY$. A structured-dependent loss function can be induced from $k_y$ by leveraging the square loss in $\bmH_y$: $\Delta(y,y'):= \| \psi(y) - \psi(y')\|^2_{\bmH_y}$. Then, given a fixed but unknown joint probability distribution $\rho$ defined on $\bmX \times \bmY$, the goal of Structured Prediction is to find an estimator $\hat{f}$ of
\begin{equation}
    f^* :=\underset{f \in \bmF(\bmX, \bmY)}{\arg \min}~ \mathbbm{E}_{x,y \sim \rho}\big[\| \psi(y) - \psi(f(x)) \| \big]\,,
\end{equation}
with the help of a training i.i.d. sample $\{(x_1,y_1),...,(x_n,y_n)\}$ drawn from $\rho$.\\

Several works \cite{cortes2005, geurts2006, Brouard_icml11, Ciliberto2016} have shown that a powerful way to tackle this problem is a two-step approach:\\
{\bf Regression of $\psi(Y)$ given $X$ (output kernel regression or surrogate problem):}\\
$\hat{h}$ estimates $h^*=\underset{h : \mathcal{X} \rightarrow \bmH_y}{\arg \min } ~ \mathbb{E}\left[\left\|h\left(x_i\right)-\psi\left(y_i\right)\right\|_{\bmH_y}^2\right]$.\\
{\bf Pre-image or decoding step:}\\
\begin{equation*}
    \hat{f}(x)=\arg \min _{y \in \mathcal{Y}}\|\hat{h}(x)-\psi(y)\|_{\bmH_y}^2.
\end{equation*}

\fl{je continue apres}

\subsection{Input Output Kernel Regression}

The method boils down to build an estimator $\hat{h}$ solving a surrogate problem with values in a linear space $\bmH_y$ instead of the structured space $\mathcal{Y}$. The advantage is that designing the hypothesis set for $\hat{h}$ and computing it is much easier.
%
Let us first recall important notions about Operator-Valued Kernels (OVKs) and vector-valued RKHSs (vv-RKHSs) \citep{Senkene1973, micchelli2005learning, carmeli2006vector, carmeli2010vector}.
%
\begin{definition}[Operator-valued kernel]
    An OVK is an application $\bmK: \bmX \times \bmX \rightarrow \bmL(\bmH_z)$, where $\bmL(\bmH_z)$ is the set of bounded linear operators on $\bmH_z$ and $\bmH_z$ is a separable Hilbert space, such that $\bmK\left(x, x^{\prime}\right)=\bmK\left(x^{\prime}, x\right)^\#$ for all $(x, x') \in \bmX^2$ -- where $\bmK\left(x^{\prime}, x\right)^\#$ denotes the adjoint of $\bmK\left(x^{\prime}, x\right)$ -- and such that for all $n \in \mathbb{N}$ and any $\left(x_{i}, \chi(z_{i})\right)_{i=1}^{n} \in(\bmX \times \bmH_z)^{n}$ we have $\sum_{i, j=1}^{n} \left\langle \chi(z_{i}), \bmK\left(x_{i}, x_{j}\right) \chi(z_{j}) \right\rangle_{\bmH_z} \geqslant 0$.
\end{definition}
%
An OVK is uniquely associated to a vv-RKHS.
%
\begin{theorem}[Vector-valued RKHS]
    Let $\bmK$ be an OVK. Then, there is a unique Hilbert space $\bmH_{\bmK} \subset \mathcal{F}(\bmX, \bmH_z)$, the vv-RKHS of $\bmK$, s.t. for all $x\in\bmX$, $\chi(z)\in \bmH_z$ and $f \in \bmH_{\bmK}$ we have $x^\prime \mapsto \bmK\left(x, x^\prime\right) \chi(z) \in \bmH_{\bmK}$, and $\langle f, \bmK\left(\cdot, x\right) \chi(z) \rangle_{\bmH} = \left\langle f(x), \chi(z) \right\rangle_{\bmH_z}$.
\end{theorem}
%
We are now equipped to describe IOKR \citep{Brouard_icml11, Brouard_ismb2016, brouard2016input} framework.
%
It consists in defining an input kernel $\bmK$ on $\bmX$ in order to set its RKHS $\bmH \subset \bmF (\bmX, \bmH_y)$ as the hypothesis space for $\hat{h}$ and use some interesting properties of OVKs, and more specifically a Representer Theorem \citep{micchelli2005learning}, to obtain the estimator minimizing the following empirical objective
\begin{equation}
    \min _{h \in \mathcal{H}} ~ \frac{1}{n} \sum_{i=1}^n\left\|h\left(x_i\right)-\psi(y_i)\right\|_{\bmH_y}^2+\lambda\|h\|_{\mathcal{H}}^2\,
\end{equation}
where $\mathcal{H}$ is the RKHS associated to an operator-valued kernel $\bmK$. In this work, we consider an identity separable kernel, i.e. of the form $\bmK\left(x, x^{\prime}\right)=k_x\left(x, x^{\prime}\right) I_{\bmH_y}$, where $k_x: \mathcal{X} \times \mathcal{X} \rightarrow \reals$ is a positive definite scalar-valued kernel on $\mathcal{X}$ associated to the RKHS $\bmH_x$. In this case, the solution $\hat{h}$ of the problem above can be computed in closed-form as $\hat{h}(x)=\sum_{i=1}^n \hat{\alpha}_i(x) \psi(y_i)$, with
\begin{equation}\label{eq:ridge_est_alpha}
    \hat{\alpha}(x)=(K_X+n \lambda)^{-1} {\kappa}_{X}^{x} = \widehat{\Omega} {\kappa}_{X}^{x}\,,
\end{equation}
where $K_X=\left(k\left(x_i, x_j\right)\right)_{i, j=1}^n \in \reals^{n \times n}$, and $\kappa_{X}^{x} = (k_x(x, x_1), \ldots,k_x(x, x_n))^\top$. The time complexity of this fitting part is dominated by the $n \times n$ matrix inversion, thus it is $\bmO\left(n^3\right)$, which can be intractable for large $n$. Hence, for a given input $x \in \bmX$, prediction $\hat{f}(x)$ is obtained by the decoding step, that boils down to the following pre-image problem
\[
    \hat{f}(x) = \underset{y \in \bmY}{\arg \min} ~ k_{y}(y, y) - 2 {{\kappa}_{X}^{x}}^T (K_{X} + n \lambda I_n)^{-1} {{\kappa}_{Y}^{y}}\,,
\]
where ${{\kappa}_{Y}^{y}} = \left(k_{y}\left(y, y_1\right), \ldots, k_{y}\left(y, y_n\right)\right)^\top$. In practice, we perform this minimisation in a discrete manner on a candidate set $\bmY_c \subseteq \bmY$ of size $n_c$. Hence, given that we want to perform predictions on a test set $X_{te}$ of size $n_{te}$, the main quantity to compute is
\begin{equation}
    \underbrace{K_{te, tr}}_{n_{te} \times n} \underbrace{\widehat{\Omega}}_{n \times n} \underbrace{K_{tr, c}^y}_{n \times n_c}\,,
\end{equation}
where $K_{te, tr} = \left(k_x(x_i^{te}, x_j)\right)_{\substack{1 \leq i \leq n_{te} \\ 1 \leq j \leq n}} \in \reals^{n_{te} \times n}$ and $K_{tr, c}^y = \left(k_{y}(y_i, y_j^c)\right)_{\substack{1 \leq i \leq n \\ 1 \leq j \leq n_c}} \in \reals^{n \times n_c}$. The complexity of decoding part is $\bmO\left(n^2 n_c\right)$, considering $n_{te} < n \leq n_c$.
%
IOKR thus suffers, like most kernel methods applied in a naive fashion, from a heavy computational cost.
%
In order to alleviate this limitation, we propose the following model, that uses sketching methods both in the input and output feature spaces to accelerate both fitting and decoding steps.

\subsection{Sketched Input Sketched Output Kernel Regression}

Let us first define some notations and quantities.
%
For any Polish space $\bmZ$, we can define a p.d. scalar-valued kernel $k_z$ uniquely associated with its RKHS $\bmH_z$.
%
We note $\chi(z) = k_z(\cdot, z)$ the canonical feature map of $k_z$ and, given a set $(z_i)_{i=1}^n$, define the sampling operator $S_Z : f \in \bmH_z \mapsto (1/\sqrt{n}) (f(z_1), \ldots, f(z_n))^\top$, its adjoint $S_Z^\# : \alpha \in \reals^n \mapsto (1/\sqrt{n}) \sum_{i=1}^n \alpha_i \chi(z_i)$ \citep{Smale_2007}, as well as the empirical covariance operator $\widehat{C}_Z = (1/n) \sum_{i=1}^n \chi(z_i) \otimes \chi(z_i) = S_Z^\# S_Z$.
%
Finally, it is easy to check that the Gram matrix rewrites as $K_Z = n S_Z S_Z^\#$.
%
Equipped with these definitions, as highlighted in \citet[Lemma~17]{Ciliberto2016}, one can show that the kernel ridge estimator $\hat{h}$ from \eqref{eq:ridge_est_alpha} can be rewritten
\begin{equation}\label{eq:ridge_est_H}
    \hat{h}(x) = S_Y^\# S_X \big(\widehat{C}_X + \lambda I\big)^{-1} \phi(x)\,,
\end{equation}
where $\phi(x) = k_x(\cdot, x)$.
%
Given orthogonal projection operators $\widetilde{P}_X$ and $\widetilde{P}_Y$ onto subspace of $\bmH_x$ and $\bmH_y$ respectively with reduced dimension, we can design an approximate estimator as follows
\begin{equation}\label{eq:tildeh_proj}
    \tilde{h}(x) = \widetilde{P}_Y S_Y^{\#}S_X \widetilde{P}_X(\widetilde{P}_X S_X^\# S_X \widetilde{P}_X + \lambda I_{\bmH_x})^{-1} \phi(x)\,.
\end{equation}
%
Basically, the idea is to replace $S_Z$ by $\widetilde{P}_Z S_Z^\#$ in order to encode dimensional reduction.
%
However, questions are: how to design the projection operators and how can we retrieve an expression of the low-rank estimator $\tilde{h}(x) = \sum_{i=1}^n \tilde{\alpha}_i \psi(y_i)$ for algorithmic purposes? \\ \\
%
As an answer to the first question, in this work, we chose to leverage sketching \citep{mahoney2011randomized, woodruff14} to obtain random projectors within the input and output feature spaces.
%
Indeed, sketching consists in approximating a feature map $\chi : \bmZ \to \bmH_z$ by projecting it thanks to a random projection operator $\widetilde P_Z \in \bmH_z \otimes \bmH_z$ defined as follows.
%
Given a random matrix $R_z \in \reals^{m_z \times n}$ and $n$ data $(z_i)_{i=1}^n \in \bmZ$, the linear subspace defining $\widetilde P_Z$ is constructed as the linear subspace generated by the span of the following $m$ random vectors
\[
    \sum_{j=1}^n (R_z)_{ij} \chi(z_j) \in \bmH_z, \quad i=1, \dots, m_Z\,.
\]
%
This random matrix is drawn from a distribution on $\reals^{m_z \times n}$, including classical examples such as sub-sampling sketches where each row is randomly drawn from the rows of the identity matrix $I_n$ (sub-sampling sketches correspond to Nystr\"{o}m approximation \citep{rudi2015less}) or Gaussian sketches where each entry are i.i.d. Gaussian random variables.
%
More precisely, given $\widetilde{C}_Z = S_Z^\# R_z^\top R_z S_Z$, $\widetilde{K}_Z = R_z K_Z R_z^\top$, $\left\{\left(\sigma_i(\widetilde{K}_Z), \tilde{\mathbf{v}}_{i}^z\right), i \in[m_z]\right\}$ the eigenpairs of $\widetilde{K}_Z$ ranked in the descending order of eigenvalues and $p_z = \operatorname{rank}\left(\widetilde{K}_Z\right)$, one can define for all $1 \leq i \leq p_z$, $\tilde{e}_i^z = \sqrt{\frac{n}{\sigma_i(\widetilde{K}_Z)}} S_Z^{\#} R_z^\top \tilde{\mathbf{v}}_{i}^z$.
%
Then, the following Proposition holds true and gives an expression of the projectors yielded by sketching.
%
\begin{proposition}\label{prop:proj_exp}
    The $\tilde{e}_i^z$s are the eigenfunctions, associated to the eigenvalues $\sigma_i(\widetilde{K}_Z)/n$, of $\widetilde{C}_Z$. Furthermore, let $\widetilde{\bmH}_z = \spn\left(\tilde{e}_1^z, \ldots, \tilde{e}_{p_z}^z\right)$, the orthogonal projector $\widetilde{P}_Z$ onto $\widetilde{\bmH}_z$ writes as
    \begin{equation}
        \widetilde{P}_Z = (R_z S_Z)^{\#} \left(R_z S_Z (R_z S_Z)^{\#}\right)^{\dagger} R_z S_Z\,,
    \end{equation}
    where $A^\dagger$ denotes the Moore-Penrose inverse of $A$.
\end{proposition}
%
\begin{remark}
    With $R_x$ a sub-sampling matrix, we recover the linear operator $L_m$ introduced in \citet{Yang_NIPS2012_621bf66d} for the study of Nystr{\"o}m approximation and its eigendecomposition. Moreover, we also recover the projection operator $P_m$ from \citet{rudi2015less} and follow the footsteps of the proposed extension ``Nystr\"{o}m with sketching matrices''.
\end{remark}
%
As a consequence, given this expression, we are able to retrieve the expansion of $\tilde{h}$ as a linear combination of the $\psi(y_i)$s.
%
\begin{proposition}\label{prop:SISOKR_exp}
    For all $x \in \bmX$, $\tilde{h}\left(x\right)=\sum_{i=1}^n \tilde{\alpha}_i\left(x\right) \psi\left(y_i\right)$ where
    \begin{equation}
        \tilde{\alpha}\left(x\right) = R_y^\top \widetilde{\Omega} R_{x} {\kappa}_{X}^{x}\,,
    \end{equation}
    with $\widetilde{\Omega} = \widetilde{K}_Y^\dagger R_y K_Y K_X R_{x}^\top (R_{x} K_{X}^2 R_{x}^\top + n \lambda \widetilde{K}_X)^{\dagger}$.
\end{proposition}
%
We here recover a classical quantity when leveraging sketching for Kernel Ridge Regression, i.e. $K_X R_{x}^\top (R_{x} K_{X}^2 R_{x}^\top + n \lambda R_{x} K_{X} R_{x}^\top)^{\dagger} R_{x} {\kappa}_{X}^{x}$ \citep{rudi2015less, Yang2017}.
%
This quantity allows to reduce the size of the matrix to invert, which is now an $m_x \times m_x$ matrix.
%
This is the main reduction that allows to reduce fitting step's complexity, thanks to the input sketching.
%
We still need to perform matrix multiplications $R_x K_X$, which can be very efficient both in time and space complexity for sketches such as sub-sampling or $p$-sparsified \citep{elahmad22} sketches, or more costly for Gaussian sketches for instance.
%
Furthermore, output sketching gives additional operations to perform, but the overall of computing $\tilde{\alpha}$ complexity can be negligeable compared to $\bmO(n^3)$ according to the sketching scheme used for both input and output kernels.
%
Finally, the purpose of output sketching is to accelerate inference.
%
In fact, the main quantity to compute now when performing predictions is
\begin{equation}
    \underbrace{K_{te, tr} R_{x}^\top}_{n_{te} \times m_{x}} \underbrace{\widetilde{\Omega}}_{m_x \times m_y} \underbrace{R_y K_{tr, c}^y}_{m_y \times n_c}\,.
\end{equation}
%
Time complexity of such an operation is $\bmO(n_c n_{te} \min(m_x, m_y))$ if $n_{te} > m_y$, and $\bmO(n_c m_y \min(m_x, n_{te}))$ otherwise.
%
We then obtain a significant complexity reduction, as we do not have any dependency in $n^2 n_c$ anymore.

==> 97-complexity.tex <==
\section{MORE DETAILS ABOUT COMPLEXITY FOR DIFFERENT SKETCHING TYPES}\label{apx:complexity}

In this section, we detail the complexity in time and space of the training and inference phase of IOKR and SISOKR algorithms for different sketching types.

\begin{table}[!ht]
\caption{Time and space complexities at training and inference for the IOKR and SISOKR algorithms with sub-sampling, $p$-sparsified ($p \in (0, 1]$) or Gaussian sketching, for a test set of size $n_{te}$  and a candidate set of size $n_c$, such that $n_{te} \leq \mx, \my < n \leq n_c$.}\vspace{0.1cm}
\begin{adjustbox}{center}
\begin{small}
\begin{tabular}{c|cc|cc}
    \toprule
    & \multicolumn{2}{c|}{Training} & \multicolumn{2}{c}{Inference} \\ 
    Method & Time & Space & Time & Space \\
    \midrule
    IOKR & $\mathcal{O}(n^3)$ & $\mathcal{O}(n^2)$ & $\mathcal{O}(n_{te} n n_c)$ & $\mathcal{O}(n n_c)$  \\
    SISOKR (sub-sampling) & $\mathcal{O}(\max(\mx, \my) n)$ & $\mathcal{O}(\max(\mx, \my) n)$ & $\mathcal{O}(n_{te} \my n_c)$ & $\mathcal{O}(\my n_c)$ \\
    SISOKR ($p$-sparsified) & $\mathcal{O}(\max(\mx, \my)^2 p n)$ & $\mathcal{O}(\max(\mx, \my) p n)$ & $\mathcal{O}(\max(n_{te}, n \my p) \my n_c)$ & $\mathcal{O}(n p \my n_c)$ \\
    SISOKR (Gaussian) & $\mathcal{O}(\max(\mx, \my) n^2)$ & $\mathcal{O}(n^2)$ & $\mathcal{O}(n \my n_c)$ & $\mathcal{O}(n n_c)$ \\
    \bottomrule
\end{tabular}
\end{small}
\end{adjustbox}
\label{table:complexities}
\end{table}
